Ionization Electron Signal Processing in Single Phase LArTPCs I. Algorithm Description and Quantitative Evaluation with MicroBooNE Simulation

We describe the concept and procedure of drifted-charge extraction developed in the MicroBooNE experiment, a single-phase liquid argon time projection chamber (LArTPC). This technique converts the raw digitized TPC waveform to the number of ionization electrons passing through a wire plane at a given time. A robust recovery of the number of ionization electrons from both induction and collection anode wire planes will augment the 3D reconstruction, and is particularly important for tomographic reconstruction algorithms. A number of building blocks of the overall procedure are described. The performance of the signal processing is quantitatively evaluated by comparing extracted charge with the true charge through a detailed TPC detector simulation taking into account position-dependent induced current inside a single wire region and across multiple wires. Some areas for further improvement of the performance of the charge extraction procedure are also discussed.

==> Makefile <==
##########################################################################
#
# $Id: Makefile,v 1.2 2010/10/29 15:06:33 slavic Exp $
#
##########################################################################
TEX = pdflatex
BIB = bibtex 
#main file
texfile = Signal_Processing_part1
#texfile = Signal_Processing_part2
#all figures
FIGS=$(wildcard figures/*.*)
#all texfiles
SECS=$(wildcard ./*.tex)
#SECS=$(wildcard sections/*.tex)

export TEXINPUTS:=$(CURDIR):$(CURDIR)/ar2estyle:$(TEXINPUTS)
export BSTINPUTS:=$(CURDIR):$(CURDIR)/ar2estyle:$(BSTINPUTS)
#export BIBINPUTS:=$(CURDIR):$(CURDIR)/ar2estyle:$(BIBINPUTS)

.PHONY: pdf
.PHONY: clean

all: pdf

pdf: $(texfile).pdf

$(texfile).pdf : $(SECS) $(texfile).tex $(texfile).bib #$(FIGS) 
	$(TEX) $(texfile)
	$(BIB) $(texfile) # compile bibliography
	$(TEX) $(texfile)
	$(TEX) $(texfile)

clean:
	@ls $(texfile).* | grep -v '.tex\|.bib' | xargs -I {} rm {}
	#@ls $(texfile).* | grep -v '.tex\|.bib' | xargs -I {} rm {}


==> types.tex <==
\section{Identification and Filtering of MicroBooNE TPC Excess Noise}\label{sec:types}

\begin{figure}[!h!tbp]
\center
\includegraphics[width=\fighalfwidth]{figs/final/noise_summary_1us.pdf}
\includegraphics[width=\fighalfwidth]{figs/final/noise_summary_2us.pdf}
\caption[excess]{Average noise magnitude in the frequency domain for 1 $\mu$s and 2 $\mu$s is 
shown. Three sources of excess noise are illustrated on the left panel: Low voltage regulator noise, 
cathode HV harmonic noise, and 900 kHz burst noise.
\textcolor{blue}{Add label for 36 and 108 kHz noise as well. And signal is already removed from this.}}
\label{excess_noise_summary}
\end{figure}

In the Sec.~\ref{sec:cold_noise}, we described the inherent noise of the
electronics that is expected to be dominated by the noise associated
with the first transistor. In MicroBooNE, we observed excess noise
beyond the expected inherent noise. 
%\fixme{MB: include plot showing
%  total noise in time domain BEFORE filtration here and add discussion
%  of how much more it is compared to expectation}.
Figure~\ref{excess_noise_summary} shows the average spectrum in
the frequency domain for U plane from an example event for 1 $\mu$s (left) and 2 $\mu$s (right) peaking time. The three
major excess noise are clearly visible.

%The TPC noise observed in MicroBooNE could come from a variety of sources,
%only the first one on the list below being unavoidable:
%\item {\bf The noise associated with amplification 
%in the first transistor of the cold electronic ASIC}: usually characterized
%  by the Equivalent Noise Charge (ENC). This noise has been described in Sec. ~\ref{sec:RC}.  
%  \item {\bf Electronic noise from the warm shaping amplifier and ADC:}
%  One of the principal objectives of low noise front end design is
%  that the readout system noise should be limited only by the noise of
%  the first transistor.  The noise of the first transistor is
%  determined by measurements and simulations (see
%  Ref~\cite{asic}). The shaping amplifier noise is small compared to
%  the first transistor noise. Overall ASIC noise is optimized against
%  power dissipation~\cite{asic}. The noise contributions from the
%  intermediate amplifier and ADC are negligible (The ASIC gain should
%  be selected so as to make the ADC quantization noise negligible).
\begin{itemize}
\item {\bf Noise induced by the low-voltage regulators:} \\
In Sec.~\ref{sec:coherent}, we describe 
the noise originating from the low-voltage regulators supplying the 
ASIC operating voltages. This noise, coherent for all the channels supplied by
each regulator, shows up at low frequency and affects all wires.


\item {\bf Noise induced by the cathode high voltage power supply:} \\
In Sec.~\ref{sec:harmonic}, we describe the noise induced on the 
anode wire plane by the voltage fluctuations in the cathode potential, 
such as ripple from the high voltage (HV) supply. This type of noise,
affects all the wires in the first induction plane, at a reduced level in the second
induction wire plane, and at an even lower level in the collection wire plane.

\item {\bf 900 kHz Burst Noise:} \\
In Sec.~\ref{sec:zig-zag}, we describe the observed burst noise with 
its frequency around 900 kHz. This type of noise has a clear  
positon dependence and has a burst nature. 
While the exact source has not 
been clearly identified, evidence is pointing towards the 
PMT high voltage supply or laser system.

%\item {\bf ASIC saturation:} \\
%As described in Sec.~\ref{sec:chirping}, a periodic saturation of the
%  ASIC has been observed in MicroBooNE. This is caused by the wire motion
%(due to liquid motion or external vibration) under the electric field. 
%The induced low-frequency current sometimes can overwhelm the bias current
%of the ASIC leading to a saturated charge amplifier. 
%
% \item {\bf Misconfigured channels:}
% As discussed in Sec.~\ref{sec:misconfig}, some channels in the first 
% induction wire plane sometimes cannot receive the proper configuration 
% command during initialization process. Instead of nominal gain, 14 mV/fC and peaking time, 2 $\mu$s
% setting, they are left at the default 4.7 mV/fC and 1 $\mu$s settings. 
% The signal in these channels are valid, but require correction for different settings.
% \item {\bf Non-Functioning channels:}
% As discussed in Sec.~\ref{sec:dead}, there are two cases of shorted wires 
% that disabled several groups of channels. Together with some dead channels these form a group 
% of non-functioning channels.
%\item {\bf Electronic noise from other circuits in the readout chain:} An
%  example would be the low frequency coherent noise from the low
%  voltage regulators supplying the ASIC operating voltages. This noise
%  was expected and a filter circuit was added to the voltage regulator
%  on the board to prevent such noise. As discussed in 
%\item {\bf Noise introduced by the wire bias power supplies:} This noise 
%was carefully determined to be negligible in MicroBooNE.
%\item {\bf Noise from the cathode HV:} The anode is highly sensitive to
%  voltage fluctuations in the cathode potential, such as from the
%  ripple from the HV supply.
\end{itemize}

In the following sections, we will describe aforementioned excess
noise in detail and compare them with
the expectation of the inherent noise to illustrate their impact on
the TPC performance. A software filter has been developed to
largely remove the excess noise with a minimal impact on signal. 

%Identification of different types of noise is obtained by using a
%combination of methods: examination of waveforms of wire signals
%recorded in the time domain, Fast Fourier Transform (FFT) of these
%waveforms and the equivalent noise charge (ENC) as a function of the
%shaping time.  
%The FFT can identify fixed continuous wave (cw)
%frequency sources of noise such as that described in
%Sec.~\ref{sec:coherent}. 
%FFT alone, particularly if used without phase
%information does not provide sufficient information. Identification of
%possible microphonics noise that caused the front-end ASIC to saturate
%(Sec.~\ref{sec:chirping}) required more complicated analysis.
%Finally, through examination of the ADC pedestal RMS on all channels
%after filtering fixed frequency noise signals, channels with very
%large unidentified residual noise and channels with very low noise can
%be characterized. 
%For each noise signal identified a software filter
%is implemented to remove the noise. 


%The noise sources identified in Sec.~\ref{sec:harmonic}
%and~\ref{sec:coherent} can be removed by hardware filters with no
%impact on the signal. The software filter is therefore an interim
%measure that demonstrates the effect of removing these sources of
%noise. Unlike a hardware filter, this cannot be done without some
%impact on the signal.

\subsection{Low Frequency Noise from Voltage Regulator}~\label{sec:coherent}

This low frequency noise is injected via the power input to the cold
ASIC. More specifically, it is due to the voltage regulator used 
to provide a stable voltage for the cold ASIC. It is pronounced at low frequencies
($\lesssim 30 \textrm{kHz}$) as shown in
Fig.~\ref{excess_noise_summary}. While the regulator noise is very
low, it still exceeds the noise of the p-channel metal-oxide
semiconductor (pMOS) input transistor. 
The source electrode of this transistor is driven
by the regulator voltage with respect to the gate electrode that is
connected to a sense wire. The resulting injected noise is thus
proportional to the wire capacitance. This noise is typically found
to be correlated across 192 channels on the same service board that
contains the same low voltage regulators. Usually,
the correlation is highest within the 48 channels covering 3 ASICs.

To subtract the regulator coherent noise, at each time tick, the
median value of the 48 channels is calculated and is used to form a
correction waveform to be subtracted from each of the 48
channels. Before subtraction, the region in the correction waveform 
corresponding to the signal is identified using threshold cut based on
ADC root mean square value. Any region above 5 times of the rms with
seven to ten time ticks extending on both sides is removed. Instead of making
the correction waveform completely zero in these regions, linear
interpolation is used. It
was also noticed that the wires on the service board's edges usually
experience a larger contribution from the coherent noise. In order to
further reduce the noise level for these edge wires, a scaling
adjustment of the correction waveform is performed during waveform subtraction. 
The scaling factor is calculated to be the
ratio of the correlation coefficient of a single channel and the average correlation
coefficient of the 48 channels. The bottom right plot of
Fig.~\ref{freq_filt} shows the waveform after the coherent noise
removal. As to be discussed in Sec.~\ref{sec:hardware}, the
regulator noise has been largely suppressed with a hardware
upgrade of the service boards.

%On April 5, 2016, a service board serving one set of channels on
%feed-through 5 was modified with an additional filter circuit to
%remove the low frequency coherent noise. The FFT of
%data taken before and after the LV filter was added is 
%shown in Fig.~\ref{fig:lvfilter}. A significant reduction in the low frequency
%component of the noise was observed that is consistent with the level
%of reduction in noise observed after the software coherent noise filter.


%\subsection{Saturation of ASICs}~\label{sec:chirping}
%
%\begin{figure}[!h!tbp]
%\center
%\includegraphics[width=\fighalfwidth]{figs/final/chirping_raw.pdf}
%\includegraphics[width=\fighalfwidth]{figs/final/chirping_filtered.pdf}
%\caption[chirp_1]{An example V-plane raw waveform after the recovery
%  of an ASIC from saturation (left). The same waveform is shown after the noise
%  filter (right).  The region corresponding to the ASIC saturation
%  (low RMS region) is identified. The distortion of the baseline after
%  the ASIC saturation is removed. The DC baseline is moved to 0 after
%  the noise filtration.}
%\label{chirping}
%\end{figure}
%
%Fig.~\ref{chirping} shows a waveform with the corresponding ASIC
%channel saturated for part of the readout window. When the ASIC channel is saturated, 
%its gain is very low and both the noise and pulser response become very small. 
%After a while, the ASIC would recover to its normal state. 
%At the beginning of the live period, there is usually a period when the baseline is distorted 
%due to the RC circuits as described in Sec.~\ref{sec:RC}.  
%This pattern would repeat itself quasi-periodically. The 
%incidence of ASIC saturation is higher when the wire bias voltage is higher and it 
%does not occur at all with zero wire bias. Direct scope measurements at the
%output of the intermediate amplifier of several U and V channels that
%periodically saturate indicates that the saturation
%effect has very low frequencies of $<$ 15 Hz, but could have different
%frequencies on different wires. 
%
%The ASIC saturation occurs when a positive current into its
%inout exceeds the bias current which keeps the ASIC input circuit 
%in equilibrium. With a large positive current the preamplifier is driven against its lower limit (near zero) and the signal gain becomes very low. This is confirmed by a dedicated bench test. The ASIC 
%bias current should be maintained as low as possible as it contributes
%to the parallel white noise (shot noise). The most likely external 
%current arises from the wire motion in the presence of electric field.
%
%A detailed calculation shows that to 
%induce a charge of greater than 50 pC
%to saturate the ASIC biased at 100 pA at frequencies in the range of
%1-20 Hz, a V-wire displacement of about 100 $\mu$m (less than the
%wire diameter) is sufficient. The wire motion by the 
%microphonic effect is not likely, since the wires are damped by the liquid so 
%that resonant excitation by a sonic wave would be greatly reduced.
%A more likely cause is convective liquid motion. Saturation is less likely 
%on shorter wires as wire displacement is proportional to $l^n$, where $l$ is wire length and n=2, 3 
%depending on the displacement force distribution.
%
%
%The cold ASIC has two bias current settings (100 pA or 500 pA). The default setting 
%of 500 pA gives about $\sim$60 electrons ENC at $1 \mu$s peaking time. During the initial MicroBooNE run, 
%the ASIC bias current was inadvertently set to 100 pA and it was observed that a large fraction 
%of channels on the induction planes (10-15\%) and a few channels on the collection 
%plane would experience quasi-periodic saturation. After resetting the ASIC bias
%current to 500 pA, the incidence of saturation was reduced to a few tens of wires.
%The remaining periodic saturation of the ASICs is time dependent and
%the more details on time dependence will be discussed in Sec.~\ref{sec:time_dep}.
%
%
%%The accurate
%%determination of the frequency of the periodic saturation from the
%%data is difficult due to the data records being short compared to the
%%saturation period (4.8 ms vs ~100 ms) 
%
%To deal with this noise, the regions of individual
%digitized signals corresponding to the saturation period are
%identified on an event-by-event basis and the baseline distortion just after recovery is removed. 
%The identification of the
%saturation region is based on finding local RMS less than 1 ADC count over within 20 time ticks. 
%The distortion of the baseline is corrected
%in the time domain. 
%The right panel of  Fig.~\ref{chirping} shows 
%the waveform after applying the noise filter and removing the baseline 
%distortion.
%
%

%As shown in Fig.~\ref{chirp_test}, a bench test was done where a current 
%sine wave at 1Hz and peak amplitude of 225pA was injected into the ASIC input 
%when input bias current is at 500pA (top panel) and in second case when input bias current 
%is at 100pA (bottom panel). In case of 500pA, no saturation was observed but when bias current is at 
%100pA, saturation was observed for half positive period of sine wave. 
%The new generation of ASICs
%has also added capability of setting 1nA and 5nA input bias current. 
%This kind of
%behavior was later identified as the result
%of a periodic saturation of the ASICs. 
%During the detector commissioning period, it was observed that the
%expected readout from some ASICs would suddenly disappear - with the
%channel noise RMS becoming very small - and then reappear after being
%off for a while. 
%This pattern keeps
%repeating with periods of the ASIC channel being live for a while and
%recording normal signals and then reverting to a no-signal state.
%Fig.~\ref{fig:chirping2} shows a measurement of the
%saturation effect from the intermediate amplifier on one of the
%V channels.
%\begin{figure}[!h!tbp]
%  \centerline{
%    \includegraphics[width=0.59\textwidth]{figs/saturation_start.pdf}
%    \includegraphics[width=0.59\textwidth]{figs/saturation_end.pdf}
%}
%\caption[Direct scope measurement of ASIC saturation effect]{Measurement of the 
%  periodic ASIC saturation effect on a V
%  channel. The start of the saturation is shown on the left when the
%  periodic pulser signals disappear from the output of the
%  intermediate amplifier and the end is on the right when they
%  reappear again~\cite{chirping2}. }
%\label{fig:chirping2}
%\end{figure}
%\begin{figure}[!h!tbp]
%\center
%\includegraphics[width=\textwidth]{figs/chirp_test.pdf}
%\caption[chirp_test]{Bench test for ASIC saturation when input bias current is at 500pA (t%op panel) and 100 pA (bototm panel). Current sine wave at 1Hz and peak amplitude of 225pA %was injected and period of saturation was observed when bias current is set at 100pA.}
%\label{chirp_test}
%\end{figure}


%\subsection{Misconfigured Channels}\label{sec:misconfig}
%
%
%The MicroBooNE TPC has a total of 8256 channels across three planes.
%The first 2400 channels are on the first induction (U) plane, the next 2400 on the 
%second induction (V) plane and remaining 3256 channels are on the collection (Y) plane,
%All these channels grouped into 516 ASICs~\cite{uboone_1} (16 channels per ASIC). 
%The settings selected for the 
%production data taking are 14 mV/fC gain and 2 $\mu$s peaking time.
%Using the pulser calibration signals, it was found that 14 ASICs (i.e, 224
%channels), do not have the correct configurations and were stuck at default
%value for the gain (4.7 mV/fC) and peaking time
%(1 $\mu$s).
%All of these channels are on the first induction (U) plane.
%The misconfiguration of the channels is believed to be caused by
%electrostatic discharge (ESD) damage of the configuration inputs on
%these ASICs. 
%%ESD is the sudden flow of electricity between two electrically 
%%charged objects caused by contact, an electrical short, or dielectric 
%%breakdown. A buildup of static electricity can be caused by 
%%tribocharging or by electrostatic induction.
%%\fixme{ESD is pretty commonly known.  Do we need to describe it?   
%%If so, then whatever this tribocharging really needs to be described.  Alternatively, take out both sentences.}
%
%
%\begin{figure}[!h!tbp]
%\center
%\includegraphics[width=\figwidth]{figs/final/FFT_misconf_corr.pdf}
%\caption[mis-con]{The average raw signal waveform for misconfigured
%channels with 1 $\mu$s peaking time and 4.7 $mV/fC$ gain (red).  
%The average raw signal waveform for same misconfigured channels 
%but after correcting to default 2 $\mu$s peaking time and 14 $mV/fC$ gain (black).
%The peak around 900 kHz in the 1~$\mu$s peaking time waveform 
%is due to the high frequency burst noise.}
%%\textcolor{red}{XQ: these figure are not good enough, need to reproduce.}}
%\label{mis-con-2}
%\end{figure}
%
%
%Since the expected electronic noise characteristics are different for 
%different peaking times, these misconfigured channels can be identified 
%by looking at the frequency content of the raw waveform. Channels with a 
%peaking time of 1$\mu$s have flatter spectra and higher amplitudes for high 
%frequency components - such as the 900 kHz burst noise - as compared 
%to the $2 \mu$s setting.  As shown in Fig.~\ref{mis-con-2}, the frequency 
%content of the 2 $\mu$s peaking time setting signal is clearly
%different from that of 1 $\mu$s.
%
%%\begin{figure}[!h!tbp]
%%\center
%%\includegraphics[width=0.49\textwidth]{figs/final/FFT_5201.pdf}
%%\includegraphics[width=0.49\textwidth]{figs/final/FFT_5000.pdf}
%%\caption[mis-con]{The raw signal waveform of 
%%the default 2 $\mu$s shaping time (left) and that for the 
%%mis-configured 1 $\mu$s shaping time (right). 
%%The peak around 900 kHz in the 1~$\mu$s shaping time waveform 
%%is due to the high frequency noise  discussed in Sec.~\ref{sec:zig-zag}.}
%%%\textcolor{red}{XQ: these figure are not good enough, need to reproduce.}}
%%\label{mis-con}
%%\end{figure}
%
%Although these channels are mis-configured, they are still usable as the
%real signals can be seen clearly apart from the electronic noise. 
%In treating these channels, their configurations are corrected
%in software  by using correct electronics response function 
%(shown in Fig.~\ref{fig:resp1}).
%
%%The new ASIC design has implemented more robust electrostatic
%%discharge protection to configuration pins based on the experience from MicroBooNE.
%%The expected electronics noise
%%characteristics are different for different shaping times.   
%%Using pulser signal
%%analysis, it was found   
%%with channels number
%%: 2016--2095, 2192--2303, and 2352--2383. 
%%ESD is the sudden
%%flow of electricity between two electrically charged objects caused by
%%contact, an electrical short, or dielectric breakdown. A buildup of
%%static electricity can be caused by tribocharging or by electrostatic
%%induction.
%%\begin{figure}[!h!tbp]
%%\center
%%\includegraphics[width=0.65\textwidth]{figs/asic.pdf}
%%\caption[asic]{Layout of the CMOS analog front end ASIC}
%%\label{asic}
%%\end{figure}
%
%%\subsection{Non-functioning Channels}~\label{sec:dead}
%%
%%
%%A study of non-functioning channels in MicroBooNE was conducted using pulser data 
%%to identify live channels and noise data to identify non-responsive channels and noisy 
%%channels. 
%%The pedestal ADC sample distribution is used to identify bad channels 
%%as follows:
%%
%%\begin{itemize}
%%\item The mean of the pedestal ADC distribution is compared to the average for
%%all three different wire planes and channels with values smaller than average (less than 1 ADC count) are identified as non-responsive.
%%\item Noisy channels are identified by comparing a channel pedestal ADC RMS above a high threshold (5 ADC counts for induction plane and 8 ADC counts for collection plane).
%%%\fixme{How is ``suitably'' determined?}
%%\item The frequency power spectrum magnitude of the digitized waveform is integrated and used to determine 
%%if channels are functioning well or not connected to a wire.  (\textcolor{red}{Brian - ?})
%%%\fixme{This sentence does not actually describe anything.}
%%\end{itemize}
%
%%As an example,  in run 3455, Event 6, there are about 433 non-functioning channels on the 
%%U plane, 98 on the V plane and 331 on the Y plane for a total of 862 non-functioning
%%channels. 
%
%The number of the non-functioning channels is largely stable (Sec.~\ref{sec:time_dep}) and the causes are summarized in Table.~\ref{tab:bad_noisy}
%
%\begin{table}[!htbp]
%\center
%\begin{tabular}{|c|l|}
%\hline
%    \# non-functioning channels & Reason \\ \hline
%    %352 & 24 misconfigured ASICS on FT1 \\
%    $\sim$20 & ASIC Saturation \\
%    96 & Six ASICS on MB 24 not connected to wires\\
%    304 & 19 ASICs due to start-up problem\\
%    126 & non-functioning channels around U-Y shorted wires with 10 noisy channels \\
%    287 & non-functioning channels around U-V shorted wires with 28 noisy channels \\
%    36  & channels that are noisy but not located near the shorted wires \\
%    \hline
%  \end{tabular}
%  \caption[Bad channels]{Summary of non-functioning channels for run 3455 Event 6 in 
%    MicroBooNE data. A total of $\sim$ 862 channels are considered 
%    non-functioning. There are small variations in the number of unresponsive 
%    channels from run to run basis.}
%  \label{tab:bad_noisy}
%  \end{table}
%
%First, as explained in 
%Sec.~\ref{sec:chirping}, there are about 20 channels that periodically suffer 
%from ASIC saturation. The exact number and location of channels 
%varies with time. Second,  six ASICs are not connected to TPC wires due to 
%an installation error. Third, about 19 ASICs  
%cannot be initialized properly inside the cold LAr (the ``start-up'' problem). 
%This issue is believed to be caused by the bandgap reference circuit in
%ASICs. A bandgap voltage reference is a temperature independent
%voltage reference circuit widely used in integrated circuits. It
%produces a fixed (constant) voltage regardless of power supply
%variations, temperature changes and circuit loading from a device.
%\fixme{So what?  How does this explain the ``start-up'' problem?}
%Lastly, there are about 126 Y channels with 116 channels having no 
%signal and 10 channels with high noises near the shorted wires between 
%V and Y plane. There are 287 U channels with 259 channels having no 
%signal and 28 channels with high noises near the shorted wires between 
%V and U plane. There are another 36 channels with high noises that are 
%not located in the aforementioned known shorted wires region.
%
%
%%The rest of this section focuses on the discussion of shorted wires in TPC. 
%%At the start of the commissioning all wire bias lines were tested and showed the
%%expected high resistance to ground (in the GOhm range). Upon application of the wire bias
%%(supplied to the signal feedthroughs~\cite{uboone_2}), three signal feedthroughs were drawing current 
%%and the operating voltage could not be sustained. Coincident with this, the noise increased 
%%on a number of U-channels by a factor of about 20 and the pulse signal was reduced by ~30\%. 
%%A single V-channel had also an anomalous response. The only plausible scenario that would 
%%explain such symptoms is that single V-wire is in contact with a number of U-wires, establishing
%%a DC contact between two different feedthroughs. The diagnosis by DC measurements was facilitated 
%%by the wire bias distribution arrangement, where each U-wires (and Y-wires) receives the bias via
%%a 22 MOhm resistor, while each V-wire has zero bias, as it is connected directly to the protection
%%diodes at the input to the front-end ASIC. Thus a measurement of the current vs. bias voltage at the
%%feedthrough indicates how many 22 MOhm resistors appear connected in parallel, i.e., how many U-wires
%%from a particular feedthrough are in contact with a V-wire. The measurement are consistent with
%%the hypothesis of about 280 U wires being shorted to ground through the V-wire. In addition, 
%%these U wires are expected to lose bias and disturb the electric field near them. As a result,
%%part of the drifting ionization electrons supposed to pass through these U wires are expected to be
%%collected by these non-functioning U wires leading to a smaller signal in the V and Y wires behind
%%them. This is confirmed by the data analysis of TPC signal. A similar incident happened at another
%%signal feedthrough. The measurement of the leakage current for the bias voltage power supply indicates
%%about 100 Y wires are shorted to ground. As a result, the ionization electrons supposed to be collected
%%by these Y wires are expected to be collected by the V wires in front leading to unipolar signals
%%in the induction V wires. This again is confirmed by the data analysis. We should note, for the ionization
%%electrons crossing these V wires, but not arriving at these shorted Y wires region, the normal bipolar
%%induction signal are seen on these V wires as expected. 
%
%
%
%%The results from these tests are listed in 
%%Table~\ref{tab:short_table}. For each bias voltage test, resistance is calculated by an average of two or 
%%three different measurements provided by the bias voltage power supply and the result is listed in the second 
%%column of Table~\ref{tab:short_table}.
%%An I-V measurement on a finer scale shows the presence 
%%of the two protection diodes by voltage offsets due to their turn-on voltage. The resultant 
%%voltage vs. current variations for select feedthroughs are plotted in Fig.~\ref{IV-curve}. 
%%Feedthrough 6 and 10 shows the ideal behavior but feedthroughs 7, 8 and 9 are abnormal and show 
%%shorted wires scenario where some of U-wires are touching one or more V-wires.
%%Also, by looking at the 
%%number of noisy wires from data and by knowing the bias circuit resistance, one can calculate 
%%the resistance in case of  wires in contact (listed in fourth column of Table~\ref{tab:short_table}) 
%%and this value can be compared with both measurements.
%
%%From all these measurement and subsequent 
%%observations, it was confirmed that a  number of U-wires are touching V-wires. A likely scenario 
%%is that a single loose (very low tension) V-wire is touching a number of V-wires. This number is in the range of 
%%50-70 and it varies with time, probably due to fluctuations in the liquid argon convection and other flow. While t%his number 
%%is not large, the wires that lose bias also disturb the electric field near adjacent wires.  The 
%%wires that lose contact with each other regain their normal signal and noise response. 
%
%
%%\begin{figure}[!htp]
%%\center
%%\includegraphics[width=\figwidth]{figs/final/IV.pdf}
%%\caption[IV-curve]{IV-Measurement Test on different feedthroughs to measure current draw vs. 
%%voltage for negative wire bias input lines.}
%%\label{IV-curve}
%%\end{figure}
%
%
%%\begin{table}[!htp]
%%\center
%%\begin{tabular}{|c|c|c|c|c|}
%%\hline
%%Resistance & Bias Voltage & IV-Measurement & U/V wires             & Wires \\
%%  (Mohm)     & Test               & Test              & Short Hypothesis &   in Contact \\ \hline
%%  FT7 & 1.13 & 1.22 & 1.13 & 39 \\
%%  FT8 & 8.36 & 8.76 & 8.45 & 3 \\
%%  FT9 & 3.36 & 3.40 & 3.25 & 10 \\ 
%%\hline
%%\end{tabular}
%% \caption[Shorted Wires]{Resistance comparison between measurements (column 2 and 3) and 
%%shorted wire hypothesis (column 3).}
%%\label{tab:short_table}
%%\end{table}
%  
%
%%\textcolor{red}{XQ: I recall there is another case of shorted wire? In addition, we need to explain the 
%%difference between 50-70 (above text) with 400 non-functioning channels due to shorted wires here.}
%
%
%\subsubsection{Time Dependence of Non-Functioning Channels}\label{sec:time_dep}
%
%In this section, we show the the time dependence of the total number of
%non-functioning channels. 
%%Production data from February through July have been analyzed. 
%The method to identify 
%these channels is explained in Sec.~\ref{sec:dead} and
%Sec.~\ref{sec:chirping}. Fig.~\ref{dead_time} shows the number of
%non-functioning channels over data taking period from February to July. Each point in the plot is averaged over
%$\sim$10 events from the given run. The behavior of non-functioning 
%channels for U and Y-plane are quite stable except around begining of March 
%for about one month period, Y-plane (cyan) had reduced number of non-functioning channels. 
%This is due to two ASICs with the ``start-up'' 
%issue that started working properly for this period of time. Also in Fig.~\ref{dead_time} it can be
%noticed that there is a decrease in non-functioning channels in V-plane
%around beginning of April.  This is correlated
%with the replacement of a faulty cryogenic pump which happened around
%same time. It has been observed that after replacing the cryogenic pump, the occurance of ASIC saturation 
%became negligible and which cause the sudden decrease in non-functioning channels. 
%
% 
%\begin{figure}[!h!tbp]
%\center
%\includegraphics[width=\figwidth]{figs/final/deadChannels_4952-6999_10794.pdf}
%\caption[dead_time]{Average number of non-functioning channels as a function of run number. 
%The average is taken over ~10 events per run. This cover the data taking period from mid 
%February to end of July.  U (blue), V (red) and Y (cyan). }
%\label{dead_time}
%\end{figure}  
%
%
%\subsection{Residual Noise Levels}~\label{sec:RMS}
%
%An example waveform before and after the entire noise filter is shown in Fig.~\ref{freq_filt} 
%(top left and bottom right). The noise level is reduced by a factor of 4--5 for the induction 
%planes and a factor of 2--3 for the collection plane.  The performance of this noise filtering is also
%shown in the 2D event displays in Figs.~\ref{evt_dis1},~\ref{evt_dis2},~\ref{evt_dis3}. The software
%noise filtering largely remove the excess of electronic noise. 
%
%\begin{figure}[!h!tbp]
%\center
%\includegraphics[width=\figwidth]{figs/final/test_3493_821_U.pdf}
%\caption[Event display]{2D event display of U-plane from run 3493 Event 41075 showing raw signal before and after noise filtering.}
%\label{evt_dis1}
%\end{figure}  
%
%\begin{figure}[!h!tbp]
%\center
%\includegraphics[width=\figwidth]{figs/final/test_3493_821_V.pdf}
%\caption[Event display]{2D event display of V-plane from run 3493 Event 41075 showing raw signal before and after noise filtering.}
%\label{evt_dis2}
%\end{figure}  
%
%\begin{figure}[!h!tbp]
%\center
%\includegraphics[width=\figwidth]{figs/final/test_3493_821_Y.pdf}
%\caption[Event display]{2D event display of Y-plane from run 3493 Event 41075 showing raw signal before and after noise filtering.}
%\label{evt_dis3}
%\end{figure}  
%
%
%Fig.~\ref{rms_before} shows the residual electronic noise  after 
%the full noise filtering is performed in terms of the ADC RMS value. 
%There are $\sim$860 channels not shown in these plots that were identified as 
%non-functioning as described in Sec.~\ref{sec:dead}. The remaining channels with anomalously high 
%ADC RMS are each examined in both the time and frequency domain. Although the observed 
%noise frequency spectra on these channels are different from the majority of  ``good'' channels, 
%good induction signals can still be seen. Therefore, we keep these channels ($\sim$84 channels in run 3455) 
%in the data analysis. 
%%Fig.~\ref{rms_after} shows the
%%calculated electronic noise in terms of the ADC RMS value after
%%removing these high RMS channels (). 
%%The raw waveforms for these channels can be seen in Ref.~\cite{web-bad-known-channels}.
%%The time-dependance of noise will be studied in detail in near future.
%
%\begin{figure}[!h!tbp]
%\center
%\includegraphics[width=0.50\figwidth]{figs/final/RMS_U_before_without_034.pdf}
%\includegraphics[width=0.50\figwidth]{figs/final/RMS_V_before_without_034.pdf}\\
%\includegraphics[width=0.50\figwidth]{figs/final/RMS_Y_before_without_034.pdf}
%\caption[ADC RMS all channels]{The residual noise level after
%  filtering in terms of the RMS value for all channels (except non-functioning channels) from run 3455 Event 6 is shown for U,
%  V, and Y planes.}
%\label{rms_before}
%\end{figure}  
%
%%\begin{figure}[!h!tbp]
%%\includegraphics[width=0.32\textwidth]{figs/final/RMS_U_after_without_034.pdf}
%%\includegraphics[width=0.32\textwidth]{figs/final/RMS_V_after_without_034.pdf}
%%\includegraphics[width=0.32\textwidth]{figs/final/RMS_Y_after_without_034.pdf}
%%\caption[ADC RMS good channels]{The residual noise level after
%%  filtering in terms of the RMS value vs. channel number after
%%  removing dead channels and known bad channels from run 3455 Event 6.}
%%\label{rms_after}
%%\end{figure} 
%
%As explained in Sec.~\ref{sec:RC}, the amount of electronics noise is
%expected to have a  dependence on the wire length. This can be seen
%already in Fig.~\ref{rms_before}.  Fig.~\ref{rms3} replot 
%the magnitude of the electronic noise with respect to the wire length
%$L$. The best-fit parameters of  fitting the data with Eq.~\eqref{eqn:rms_fit1}
%are
%%A fit to the noise
%%level as a function of wire length 
%%\begin{equation}
%%\begin{aligned}
%  %\textrm{Noise}_\textrm{RMS}~\textrm(ADC) = 1.152 + 0.00184 \times L (cm).
%%  \textrm{Noise}_\textrm{RMS}~\textrm(ADC) = \sqrt{A^2 + {(B*L(cm) + C)^2}}
%%  \label{eqn:rms_fit1}
%%\end{aligned}  
%%\end{equation} 
%%with fit parameters
%$A = 0.4616$ ADC, $B = 0.19$ ADC/m and $C = 1.07$ ADC. Wire capacitance can be calculated using Fig.~\ref{fig:enc_cin}, which shows the variation of ENC with input capacitance and from fit parameters of Eq.~\ref{eqn:rms_fit1}, and is found to be about $(23 \pm 2)$~pF/m.
%
%The noise level in terms of ADC is converted to the equivalent noise charge (ENC) as follows:
%\begin{equation}
%  \frac {ENC} {ADC} =  \frac{2000~mV}{4096~\textrm{ADC}} \times \frac{1~fC}{14~mV} \times \frac {1}{1.1}\times \frac{\textrm{ 6241~electrons}}{fC} = 198~\textrm{electrons}.
%  \label{eqn:adctoenc}
%\end{equation}
%
%%Dependance of ENC on wire length and hence wire capacitance can be clearly seen from Fig.~\ref{rms3}.
%%Using Fig.~\ref{fig:enc_cin}, which shows the variation of ENC with input capacitance and fit from Eq.~\ref{eqn:rms_fit1}, 
%%we can calculate the different components of electronics noise and input wire capacitance value.
%%Each fit parameter in Eq.~\ref{eqn:rms_fit1} is related to different noise contribution. Fit parameter ``A'' 
%%doesn't depend on wire length and corresponds to digitization noise with ENC contribution of $\sim$ 90 electrons. 
%%Similarly, ``C'' doesn't depend on wire length and corresponds to detector and motherboard parasitic noise with ENC contribution of $\sim$ 212 electrons.
%%Parameter ``B'' clearly depends on wire length and corresponds to wire capacitance of $\sim (23 \pm 2)$~pF/m, using Fig.~\ref{rms3} and Fig.~\ref{fig:enc_cin}.  
%
%The factors of 14 mV/fC and 1.1 are the gain of the cold ASIC and
%the intermediate amplifier, respectively.  Therefore, the nominal ENC
%for the induction wires is about 430 electrons for longest wires. This is the lowest
%noise achieved by any LArTPC greater than 100 tons to date. Fig.~\ref{rms_run} shows 
%stability of the ADC RMS for same length wires (longest wires for induction planes and all collection plane wires) over 
%run period from February through July with each point in plot is average over $\sim$ 10
%events from given run. 
%
%%From Eq.~\ref{eqn:rms_fit1} and Eq.~\ref{eqn:adctoenc}, the expected ENC
%%on a wire of 12~m - which corresponds to an input capacitance of 220 pF - 
%%with a 2 $\mu$s shaping time would be 610 electrons, which is in excellent agreement with the
%%test-stand measurements at BNL of the ASIC in the cold as shown in
%%Fig.~\ref{fig:enc_peaking}.
%
%\begin{figure}[!h!tbp]
%\center
%\includegraphics[width=\figwidth]{figs/final/RMSvsLength_after_without_034.pdf}
%\caption[Residual noise vs wire length]{The noise level in terms of the RMS value and ENC is plotted with respect to the wire length. The vertical band in magenta are all of the Y-plane wires which have the same length and the vertical green band at the right most end of the plot is all longest wires from U and V-planes.}
%\label{rms3} 
%\end{figure}   
%
%\begin{figure}[!h!tbp]
%\center
%\includegraphics[width=\figwidth]{figs/final/RMSvsRun_4952-6999_10794.pdf}
%\caption[RMS_Run]{Average of ADC root mean square for constant length U, V and Y wires as a function of run number. The average is taken over ~10 events per run. This cover the data taking period from mid February to end of July, before summer shutdown. U (blue), V (red) and Y (cyan) }
%\label{rms_run} 
%\end{figure}   
%
%

\subsection{The HV Power Supply Noise}~\label{sec:harmonic}

%\begin{figure}[!h!tbp]
%\center
%\includegraphics[width=0.95\textwidth]{figs/HV_noise_2.png}
%\caption[HV_noise]{A sample of waveforms dominated by 
%HV power supply noise on the U and V wires and negligible on the Y wires.}
%\label{HV_noise}
%\end{figure}

As shown in Fig.~\ref{excess_noise_summary}, the examination of the
noise on U-plane channels in the frequency domain
reveals a series of single frequency lines that appear to be odd
harmonics of the 36 kHz ripple frequency of the HV power supply.  The
two main (highest and second highest) single frequency noise
components corresponds to 36 kHz and 108 kHz, with the other single
frequency component's amplitude being much smaller. The peak magnitude
of this harmonic noise in the first induction plane ``U'' is about 15
ADC counts. The magnitude of this
harmonic noise is attenuated in the second induction plane ``V'' by
about a factor of three due to the shielding by U-wires, and the noise
on ``Y'' collection wires is further attenuated to a negligible level
by shielding of both U and V wires.

In order to understand how sensitive the anode plane is to tiny 
potential variations at the cathode 2.5 meters away, a simple estimation
can be made. For a 2.5 m wire length with a sense wire capacitance of $\sim$20 $fF/m$, the induced charge 
would be $\sim$0.05 $fC/ mV$, resulting in $\sim$300 e$^-$/mV. The expected peak 
amplitude of the waveform is $\sim 15$ ADC counts which corresponds to a charge of 
$\sim$0.5 fC. Therefore, only about 10 mV at the cathode 
can produce the observed noise, or about 5 parts in $10^8$ of the drift voltage.


%In order to understand how sensitive the anode plane is to tiny 
%potential variations at the cathode 2.5 meters away, a simple estimation
%is made in the following: 
%\begin{itemize}
%\item The single sense wire capacitance to cathode (2.5 m drift, 3 mm wire
%  spacing) is $\sim$20 $fF/m$.
%\item Assuming a 2.5 m wire length, the induced charge would be
%  $\sim$0.05$fC/ mV$, resulting in $\sim$300 e$^-$/mV.  
%\item The expected peak
%  amplitude of the waveform is $\sim 15$ ADC counts corresponding to 
%   $\sim$0.5 fC. 
%\item Therefore, only about 10 mV at the cathode
%  can produce the observed noise, or about 5 parts in $10^8$ of the
%  drift voltage.
%\end{itemize}

In the software filter, the harmonic noise is directly removed from
the frequency domain.
%The hardware filter
%solution currently under way by the HV and electronics teams, is to
%add an additional stage of low pass filtering between the HV supply
%and the cathode (an additional ``beanpot'').
Fig.~\ref{freq_filt} shows the effect of noise filters on the
single-frequency noise components. The top left panel shows an example
waveform from a U-plane where it is difficult to
differentiate the signal from the noise. The top right panel is the
same waveform after filtering out the 36 kHz noise and the bottom left
panel is after filtering out both the 36 kHz and 108 kHz noise. Two
peaks from signals can be clearly identified after the noise
filtration. As to be discussed in Sec.~\ref{sec:hardware}, during the detector hardware 
upgrades in summer shutdown, the HV
power supply noise is later completely removed after installation of
an additional hardware filter in the high voltage cable connecting to the
TPC cathode.

\begin{figure}[!h!tbp]
\center
\includegraphics[width=\fighalfwidth]{figs/final/raw_signal_new.pdf} 
\includegraphics[width=\fighalfwidth]{figs/final/raw_signal_after_36_new.pdf} 
\includegraphics[width=\fighalfwidth]{figs/final/raw_signal_after_both_new.pdf} 
\includegraphics[width=\fighalfwidth]{figs/final/raw_signal_after_full_filter_new.pdf}
\caption[freq_filt]{A U-plane waveform from data (top left),
%(Channel 1513) from data Run 3455 (top left), 
  the same waveform after filtering out 36 kHz noise
  (top right), and the same waveform after filtering out both 36 kHz and
  108 kHz noise components (bottom left) are shown. The waveform after full 
  software noise filtering chain (bottom right). 
  36 and 108 kHz noise is due to the HV supply ripple, 
  and this noise is about $\sim$3 times lower on the V plane 
  and negligible on the Y plane.}
\label{freq_filt}
\end{figure} 



\subsection{900 kHz Noise (Burst Noise)}~\label{sec:zig-zag}

\begin{figure}[!h!tbp]
\center
\includegraphics[width=\figwidth]{figs/final/zigzag_time_domain-1.pdf}
\includegraphics[width=\figwidth]{figs/final/zigzag_time_domain-2.pdf}
\caption[zigzag_time_domain]{The ``900 kHz noise'' of a V-plane channel is 
shown. Blue highlighted region is identified burst noise region and red is actual channel waveform.}
\label{zigzag_time_domain}
\end{figure}


%\begin{figure}[!h!tbp]
%\center
%\includegraphics[width=\figwidth]{figs/final/FFT_1us_2us.pdf}
%\caption[mis-con]{The raw signal waveform of 
%the default 2 $\mu$s peaking time (black) and that for the 
%mis-configured 1 $\mu$s peaking time (red). 
%The peak around 900 kHz in the 1~$\mu$s peaking time waveform 
%is due to the high frequency burst noise.}
%%\textcolor{red}{XQ: these figure are not good enough, need to reproduce.}}
%\label{mis-con}
%\end{figure}


The waveforms with the ``900 kHz noise'' are shown in
Fig.~\ref{zigzag_time_domain}. Blue highlighted region is identified
as burst noise region and is identified using simple selection
criteria, where we look for any two consecutive time ticks varying
between above and below baseline alternatively, and with this pattern
repeating for at-least 5 time ticks. Also, the absolute value of the
difference in ADC counts measured between two consecutive ticks must
be larger 3 ADCs.  The oscillation (or ringing) has a mean period of
$\sim$ 1.1 $\mu$s corresponding to $\sim$ 900 kHz, evident in the
frequency spectrum in Fig.~\ref{excess_noise_summary}.  The bursts of
this noise are intermittent with the amplitude varying in time. This
noise has been observed on the wires concentrated at one corner for
the detector.  The anti-aliasing filter can be used to suppress it by
using a longer peaking time.  As expected, this noise is prominent
with 1 $\mu$s peaking time, but almost absent with the 2 $\mu$s
peaking time. This high frequency noise can also be removed by
applying a low-pass frequency filter in software. Given that this noise is negligible
with the 2 $\mu$s peaking time, there is no need to apply the low-pass
software filter in the nominal running configuration. Although the
exact origin of this noise has not been identified, current evidence
is pointing to the power switching circuits related to either PMT high
voltage power supply or the calibration laser interlock system. The
impact of this noise on the signal processing is negligible.


%As shown in Fig.~\ref{chirp_test}, a bench test was done where a current 
%sine wave at 1Hz and peak amplitude of 225pA was injected into the ASIC input 
%when input bias current is at 500pA (top panel) and in second case when input bias current 
%is at 100pA (bottom panel). In case of 500pA, no saturation was observed but when bias current is at 
%100pA, saturation was observed for half positive period of sine wave. 
%The new generation of ASICs
%has also added capability of setting 1nA and 5nA input bias current. 
%This kind of
%behavior was later identified as the result
%of a periodic saturation of the ASICs. 
%During the detector commissioning period, it was observed that the
%expected readout from some ASICs would suddenly disappear - with the
%channel noise RMS becoming very small - and then reappear after being
%off for a while. 
%This pattern keeps
%repeating with periods of the ASIC channel being live for a while and
%recording normal signals and then reverting to a no-signal state.
%Fig.~\ref{fig:chirping2} shows a measurement of the
%saturation effect from the intermediate amplifier on one of the
%V channels.
%\begin{figure}[!h!tbp]
%  \centerline{
%    \includegraphics[width=0.59\textwidth]{figs/saturation_start.pdf}
%    \includegraphics[width=0.59\textwidth]{figs/saturation_end.pdf}
%}
%\caption[Direct scope measurement of ASIC saturation effect]{Measurement of the 
%  periodic ASIC saturation effect on a V
%  channel. The start of the saturation is shown on the left when the
%  periodic pulser signals disappear from the output of the
%  intermediate amplifier and the end is on the right when they
%  reappear again~\cite{chirping2}. }
%\label{fig:chirping2}
%\end{figure}
%\begin{figure}[!h!tbp]
%\center
%\includegraphics[width=\textwidth]{figs/chirp_test.pdf}
%\caption[chirp_test]{Bench test for ASIC saturation when input bias current is at 500pA (t%op panel) and 100 pA (bototm panel). Current sine wave at 1Hz and peak amplitude of 225pA %was injected and period of saturation was observed when bias current is set at 100pA.}
%\label{chirp_test}
%\end{figure}

%\subsection{Software Filtering of Excess TPC Noise}



\subsection{Impact of Noise Filtering on Signal}


==> units.tex <==
% This holds some short-hand definitions of macros based on siunitx to
% help keep consistency of quantities and units.

% see
%  http://ctan.org/pkg/siunitx
%  http://mirrors.ctan.org/macros/latex/contrib/siunitx/siunitx.pdf

% Examples:
%  % angles
%  \ang{1.5} off-axis
%
%  % just a unit
%  \si{\kilo\tonne}
%
%  % with a value:
%  \SI{10}{\mega\electronvolt}
%
%  % range of values:
%  \SIrange{60}{120}{\GeV}
%
%  % some number, let LaTeX deal with commas, etc
%  \num{32600}

\usepackage{siunitx}

% some shorthand notation
\DeclareSIUnit \mm {\milli\meter}
\DeclareSIUnit \cm {\centi\meter}
\DeclareSIUnit \us {\micro\second}
\DeclareSIUnit \ms {\milli\second}
\DeclareSIUnit \pA {\pico\ampere}
\DeclareSIUnit \pC {\pico\coulomb}
\DeclareSIUnit \fC {\femto\coulomb}
\DeclareSIUnit \fF {\femto\farrad}
\DeclareSIUnit \pF {\pico\farrad}
\DeclareSIUnit \mV {\milli\volt}
\DeclareSIUnit \kV {\kilo\volt}
\DeclareSIUnit \V {\volt}
\DeclareSIUnit \GOhm {\giga\ohm}
\DeclareSIUnit \MOhm {\mega\ohm}
\DeclareSIUnit \ton {\tonne}
\DeclareSIUnit \kton {\kilo\tonne}
\DeclareSIUnit \kt {\kilo\tonne}
\DeclareSIUnit \Mt {\mega\tonne}
\DeclareSIUnit \eV {\electronvolt}
\DeclareSIUnit \keV {\kilo\electronvolt}
\DeclareSIUnit \MeV {\mega\electronvolt}
\DeclareSIUnit \GeV {\giga\electronvolt}
\DeclareSIUnit \km {\kilo\meter}
\DeclareSIUnit \kW {\kilo\watt}
\DeclareSIUnit \MW {\mega\watt}
\DeclareSIUnit \MHz {\mega\hertz}
\DeclareSIUnit \kHz {\kilo\hertz}
\DeclareSIUnit \mrad {\milli\radian}
\DeclareSIUnit \year {year}
\DeclareSIUnit \POT {POT}
\DeclareSIUnit \sig {$\sigma$}
\DeclareSIUnit\parsec{pc}
\DeclareSIUnit\lightyear{ly}
\DeclareSIUnit\foot{ft}
\DeclareSIUnit\ft{ft}
% for a bare kt-year
\def\ktyr{\si[inter-unit-product=\ensuremath{{}\cdot{}}]{\kt\year}\xspace}
\def\Mtyr{\si[inter-unit-product=\ensuremath{{}\cdot{}}]{\Mt\year}\xspace}
\def\msr{\si[inter-unit-product=\ensuremath{{}\cdot{}}]{\meter\steradian}\xspace}
\def\ktMWyr{\si[inter-unit-product=\ensuremath{{}\cdot{}}]{\kt\MW\year}\xspace}

\newcommand{\SIadj}[2]{\SI[number-unit-product = -]{#1}{#2}}
% Adjective form of some common units
% "the 10-kt detector"
\newcommand{\ktadj}[1]{\SIadj{#1}{\kt}}
% "the 1,300-km baseline"
\newcommand{\kmadj}[1]{\SIadj{#1}{\km}}
% "a 567-keV endpoint"
\newcommand{\keVadj}[1]{\SIadj{#1}{\keV}}
% "Typical 20-MeV event"
\newcommand{\MeVadj}[1]{\SIadj{#1}{\MeV}}
% "Typical 2-GeV event"
\newcommand{\GeVadj}[1]{\SIadj{#1}{\GeV}}
% "the 1.2-MW beam"
\newcommand{\MWadj}[1]{\SIadj{#1}{\MW}}
% "the 700-kW beam"
\newcommand{\kWadj}[1]{\SIadj{#1}{\kW}}
% "the 100-tonne beam"
\newcommand{\tonneadj}[1]{\SIadj{#1}{\tonne}}
% "the 4,850-foot depth beam"
\newcommand{\ftadj}[1]{\SIadj{#1}{\ft}}
%

% Mass exposure, people like to put dots between the units
% \newcommand{\ktyr}[1]{\SI[inter-unit-product=\ensuremath{{}\cdot{}}]{#1}{\kt\year}}
% must make usage of \ktyr above consistent with this one before turning on

% Beam x mass exposure, people like to put dots between the units
\newcommand{\ktmwyr}[1]{\SI[inter-unit-product=\ensuremath{{}\cdot{}}]{#1}{\kt\MW\year}}


